Downlink Analysis and Evaluation of Multi-Beam LEO Satellite Communication in Shadowed Rician Channels

The extension of wide area wireless connectivity to low-earth orbit (LEO) satellite communication systems demands a fresh look at the effects of in-orbit base stations, sky-to-ground propagation, and cell planning. A multi-beam LEO satellite delivers widespread coverage by forming multiple spot beams that tessellate cells over a given region on the surface of the Earth. In doing so, overlapping spot beams introduce interference when delivering downlink concurrently in the same area using the same frequency spectrum. To permit forecasting of communication system performance, we characterize desired and interference signal powers, along with SNR, INR, SIR, and SINR, under the measurement-backed Shadowed Rician (SR) sky-to-ground channel model. We introduce a minor approximation to the fading order of SR channels that greatly simplifies the PDF and CDF of these quantities and facilitates statistical analyses of LEO satellite systems such as probability of outage. We conclude this paper with an evaluation of multi-beam LEO satellite communication in SR channels of varying intensity fitted from existing measurements. Our numerical results highlight the effects satellite elevation angle has on SNR, INR, and SINR, which brings attention to the variability in system state and potential performance as a satellite traverses across the sky along its orbit.

==> sec-simulation-results.tex <==
\input{tab/tab-sim-params.tex}

\input{tab/tab-sr-params.tex}

\section{Performance Evaluation of a 20 GHz Multi-Beam LEO Satellite System\\in Shadowed Rician Channels} \label{sec:simulation-results}
In this section, we simulate a 20 GHz (Ka-band) multi-beam \leo satellite communication system and evaluate the impact various system parameters have on key performance metrics, namely \gsnr, \ginr, and \gsinr.
A summary of parameters used for simulation is listed in \tabref{tab:sim-params}, most of which are based on \cite{3gpp38811,3gpp38821} published by 3GPP on the topic of satellite communication.
We simulate a satellite at an altitude of $H = 600$ km equipped with 19 spot beams; each steered toward the center of its cell on the ground.
Cells are tessellated in a hexagonal fashion with a cell radius of 10 km.
% Each cell has a radius of 10 km, and the cells are tessellated in a hexagonal fashion.
The gain delivered by the $i$-th spot beam to a user on the ground we model as steerable dish antennas with gain pattern \cite{3gpp38811} 
\begin{align}
	G_i(\phi,\theta) = 
	\begin{dcases}
		1, & \zeta = 0^\circ \\
		4 \bars{\frac{J_1(ka \sin \zeta)}{ka \sin \zeta}}^2, & 0^\circ < |\zeta| \leq 90^\circ
	\end{dcases}
	\label{eq:beam}
\end{align}
where $\zeta = \arccos\parens{\cos \phi \cdot \cos \theta}$ is the absolute angle off from the antenna boresight, $J_1(\cdot)$ is the first-order Bessel function of the first kind, $a$ is the radius of the dish antenna, $k = 2 \pi / \lambda$ is the wave number, and $\lambda$ is the carrier wavelength. 
We model ground users as very small aperture terminals (VSAT) mounted on rooftops or vehicles with a maximum receive antenna gain of $39.7$ dBi, the noise figure of $1.2$ dB, and antenna temperature of $150$ K (i.e., $G/T = 15.9$ dB/K) \cite{3gpp38821}. 
We assume ground users track their serving satellite to offer maximum receive gain.

\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth,height=0.26\textheight,keepaspectratio]{fig/dish-pattern}
	\caption{The normalized beam pattern of each high-gain dish onboard the satellite as a function of angle off boresight $\zeta$.}
	\label{fig:dish-pattern}
\end{figure}

We consider \sr channels with three levels of shadowing---light, average, and heavy---whose parameters $(b,m,\Omega)$ are fitted from measurements in \cite{newsimple} and are shown in \tabref{tab:sr-params}.
Each onboard transmitter supplies $4$ dBW/MHz of power, and we simulate the system over a bandwidth of $400$ MHz. 
Path loss is modeled as the combination of free-space path loss and atmospheric attenuation as \cite{3gpp38811}
\begin{align}
	\mathrm{PL}(d,f_{\mathrm{c}}, \epsilon) = \mathrm{PL}_{\mathrm{FS}}(d, f_c) + \mathrm{PL}_{\mathrm{g}}(f_{\mathrm{c}}, \epsilon)
\end{align}
which is a function of propagation distance $d$, carrier frequency $f_{\mathrm{c}}$, and satellite elevation angle $\epsilon$.
Here, free-space path loss (in dB) is modeled as \cite{3gpp38811}
\begin{align}
	\todB{\mathrm{PL}_{\mathrm{FS}}(d, f_{\mathrm{c}})} = 32.45 + 20 \log_{10}(f_{\mathrm{c}}) + 20 \log_{10}(d)
\end{align}
which captures clutter loss and additional large-scale shadowing
and absorption by atmospheric gases is modeled as \cite{itur_618_13,iturp676}
\begin{align}
	\mathrm{PL}_{\mathrm{g}} (f_{\mathrm{c}}, \epsilon) = \frac{A_{\mathrm{zen}}(f_{\mathrm{c}})}{\sin \epsilon}
\end{align}
where $A_{\mathrm{zen}}$ is a zenith attenuation which is given as $A_{\mathrm{zen}} = 0.9$ at frequency $20$ GHz \cite{iturp676}.


%\begin{align}
%P = \frac{L+N}{L}= 1 + \frac{N}{L}
%\end{align}

%Satellite channel measurements have been collected and fitted to the \sr distribution, and parameter values are set to indicate various realistic levels of shadowing \cite{loo,newsimple,sr_simul}; these papers suggest the shadowing parameters 
%to categorize shadowing conditions from which engineers can simulate, evaluate, and tailor satellite communication systems. 
%We choose three parameter sets representing light, average, or heavy shadowing levels as in \tabref{table:channel} for evaluation. 
%Note that the shadowing parameters in \tabref{table:channel} are denoted with tildes since they correspond to measurements of \textit{received signal power} rather than to the channel itself.
%These received power shadowing parameters can be mapped to channel parameters $b$ and $\Omega$ by scaling $\tilde{b}$ and $\tilde{\Omega}$ according to \thmref{thm:scaled-ssr}. Also, the average received power under each shadowing level can be derived based on \thmref{thm:m-integer} and \corref{cor:mean-ssr} if the fading order $\tilde{m}$ is an integer. 
%
%
%
%Based on the shadowing level parameters given in \tabref{table:channel}, 
%we highlight satellite channel characteristics. The channel has \los and \nlos components, and each has random fluctuations. Under an environment without random channel modeling, we consider only \los component without random fluctuations, and the received signal only experiences losses by the path distance. 
%When randomness exists in the channel, both of \los and \nlos terms randomly fluctuate and are faded. 
%In lighter shadowing, it is expected that more of the signal power is tends to be delivered via \los component, and the signal is less faded. 
%Under heavy shadowing, the \nlos component dominates, and the signal is more scattered and faded. 
%We point out that the shadowing levels we have in this paper do not fully describe satellite channel variations. 
%Instead, they are just representative sets for analyses and evaluations. 
%One can manipulate channel parameters by adjusting the \los to \nlos power ratio $\frac{\Omega}{2\cdot b}$ depending on the environment setting and the fading order $m$, and realize the \sr channel using the \pdf, \cdf, and their characteristics provided in this paper. 



\subsection{Effect of Elevation Angle on Antenna Gain}

\begin{figure*}[t]
	\centering
	\subfloat[Elevation of $\epsilon = 90^\circ$.]{\includegraphics[width=0.49\linewidth,height=\textheight,keepaspectratio]{fig/ant_gain_90_20g}
		\label{fig:gain-90}}
	\hfill
	\subfloat[Elevation of $\epsilon = 45^\circ$.]{\includegraphics[width=0.49\linewidth,height=\textheight,keepaspectratio]{fig/ant_gain_45_20g}
		\label{fig:gain-45}}\\
	\caption{Delivered antenna gain as a function of ground user position for a satellite elevation angle of (a) $\epsilon = 90^\circ$ and (b) $\epsilon = 45^\circ$. Delivered beam gain distorts to a more elliptical shape at lower elevations, leading to less defined cell boundaries.}
	\label{fig:gain-elevation}
\end{figure*}


We begin our system evaluation by highlighting the effect of satellite elevation angle on antenna gain delivered to ground users in \figref{fig:gain-elevation}.
In \figref{fig:gain-90}, the satellite is directly overhead the origin at an elevation of $\epsilon = 90^\circ$.
Plotting the observed antenna gain as a function of ground user location reveals the hexagonal arrangement of our cells; shown here are the six cells surrounding the centermost cell located at the origin.
The observed spot beam gain is circular, which produces cell boundaries that are well-defined.
Maximum gain is around $38.5$ dB with cell-edge users losing around $3$ dB of gain for this particular cell radius.
A user's distance from the center of its cell is a good indicator of the antenna gain it enjoys.
As elevation is decreased to $45^\circ$ (an increased presence along the $x$ axis), the satellite is closer to the horizon and the observed spot beam gain becomes more elliptical as it projects onto the surface of the Earth.
Consequently, the beam gain elongates along the $x$ dimension and tightens along the $y$ dimension. 
Cell boundaries are no longer as well-defined and user distance from the center of the cell is no longer a clear indicator for delivered beam gain. 
For instance, users in region A, enjoy near-maximal beam gain even though they are at the cell edge, which can in fact be higher than what was observed when the satellite was overhead at $\epsilon = 90^\circ$.
Users in region B, also at the cell edge, see around $2$--$3$ dB less beam gain.
All these takeaways can be extrapolated for elevations between $45^\circ$ and $90^\circ$ and, through symmetry, beyond to $135^\circ$.
\edit{Users are associated with cells based on location, not max gain.}

%The delivered antenna gain based on the ground user's location per satellite elevation angle is presented by simulations. 
%\figref{fig:gain-elevation} shows the heatmap of delivered antenna gain as a function of ground user location with the satellite's elevation angle of $90^\circ$ (\figref{fig:gain-90}) and $45^\circ$ (\figref{fig:gain-45}). 
%For the sake of discussion, let us consider only the center cell and the six surrounding cells.
%With the elevation angle $\epsilon = 90^\circ$, the delivered antenna gain is decreased as the distance from the cell center on the ground is increased. 
%On the other hand, with the elevation angle $\epsilon = 45^\circ$, the delivered antenna gain is decreased as a user moves from the center along the $y$-axis; while it is not much reduced when a user moves along with $x$-axis. 
%In other words, not every user around cell boundaries experiences a similar level of delivered antenna gain at $\epsilon=45^\circ$. A relatively lower antenna gain is delivered to area B than to area A in \figref{fig:gain-45}. 
%Therefore, the cell shape is no longer a circle but an oval, and the distance from the cell center does not dictate the delivered gain. 
%%Note that the satellite location is projected onto the $x$-axis on the ground by the setting we have $\Phi = 0^\circ$, and the exact position is determined based on the elevation angle of the satellite. Therefore, as the elevation angle goes off from $90^\circ$, the ellipse grows in the direction of $x$-axis. 

\subsection{SNR Distribution}

\begin{figure*}[!t]
	\centering
	\subfloat[Elevation of $\epsilon = 90^\circ$.]{\includegraphics[width=0.49\linewidth,height=\textheight,keepaspectratio]{fig/heat_90_snr}
		\label{fig:snr-90}}
	\hfill
	\subfloat[Elevation of $\epsilon = 45^\circ$.]{\includegraphics[width=0.49\linewidth,height=\textheight,keepaspectratio]{fig/heat_45_snr}
		\label{fig:snr-45}}\\
	\caption{Received \gsnr as a function of user location under light shadowing for a satellite elevation angle of (a) $\epsilon = 90^\circ$ and (b) $\epsilon = 45^\circ$. User location is a good indicator for trends in \gsnr, but \sr channel stochastics can lead to deep fades even near the center of the cell.}
	\label{fig:snr-elevation}
\end{figure*}

Now, instead of considering delivered beam gain, which is solely a function of cell placement and user location, we examine \gsnr as a function of user location in the presence of light shadowing (see \tabref{tab:sr-params}) in \figref{fig:snr-elevation}.
We again consider elevations of $\epsilon = 90^\circ$ and $\epsilon = 45^\circ$ in \figref{fig:snr-90} and \figref{fig:snr-45}, respectively.
The beam patterns observed before are apparent here at a high level as trends in \gsnr follow those seen in \figref{fig:gain-elevation}.
Users in region A tend to enjoy higher \gpsnr than those in region B.
In both cases, \gsnr tends to be higher near the center of each cell, with best-case users enjoying \gpsnr around $15$ dB up to even $20$ dB.
Notice that \gpsnr observed for $\epsilon = 90^\circ$ are around $2$--$3$ dB higher than for $\epsilon = 45^\circ$; this is attributed to increased distance (and hence path loss) at lower elevation angles.
Users, especially at the cell edge, can enjoy the upper tail of the \sr channel distribution but more prominently, we see that shadowing can cause deep fades.
Naturally, since users close to the center of the cell enjoy higher $\lsnr$, they are more robust to these deep fades but are not exempt from such.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth,height=0.27\textheight,keepaspectratio]{fig/frf1_90_45_snr}
    \caption{The \cdf of \gsnr for various shadowing levels and elevations of $\epsilon = 90^\circ$ and $\epsilon = 45^\circ$.} %SNR distribution on the ground per elevation angle under various shadowing.}
    \label{fig:snr-cdf}
\end{figure}

In \figref{fig:snr-cdf}, we plot the \cdf of \gsnr for various levels of shadowing and for $\epsilon = 90^\circ$ and $\epsilon = 45^\circ$.
Here, the \cdf is taken across user locations within a cell and over channel realizations.
Light shadowing conditions produce the highest \gsnr distribution, with median users enjoying around $\msnr = 14$ dB at $\epsilon = 90^\circ$ and just over $\msnr = 11$ dB at $\epsilon = 45^\circ$.
Worst-case users in light shadowing can suffer from deep fades that result in \gpsnr falling well below $5$ dB at both elevations.
As shadowing intensifies, the \gsnr distribution shifts leftward---a shift of about $12$ dB in the median from light to heavy shadowing---from which it is clear that shadowing level can severely impact performance.
Heavier shadowing produces a heavier lower tail and more variance overall. 
Since shadowing is independent of elevation angle, there is a consistent $2$--$3$ dB gap in distribution for all three shadowing levels.
Again, interpolation between distributions can be used when considering elevations between $45^\circ$ to $135^\circ$.




%\begin{figure*}[!t]
%    \centering
%    \subfloat[SNR distribution per shadowing level at $\epsilon = 90^\circ$. ]{\includegraphics[width=0.5\linewidth]{fig/frf1_90_snr} \hfill
%        \label{fig:snr-cdf-a}}
%    \subfloat[SNR distribution per shadowing level depending on the elevation angle.]{\includegraphics[width=0.5\linewidth]{fig/frf1_90_45_snr}\hfill
%        \label{fig:snr-cdf-b}}\\
%    \caption{The \cdf of \gsnr for various shadowing levels and elevations of $\epsilon = 90^\circ$ and $\epsilon = 45^\circ$.} %SNR distribution on the ground per elevation angle under various shadowing.}
%    \label{fig:snr-cdf}
%\end{figure*}

%\figref{fig:snr_sh_el} displays SNR distribution per shadowing level and elevation angle. 
%In the figure, 'None' refers to the case where no random channel is modeled, i.e., only \los component exists without random shadowing. 'Light', 'Average', and 'Heavy' refer to the corresponding level of shadowing described in \tabref{table:channel}. 
%We look at the \snr distribution per shadowing level at the elevation angle of $90^\circ$ in \figref{fig:snr_sh}. 
%\snr without random channel ranges around $10$ dB to $13$ dB, and we notice that the delivered \snr at cell boundaries is only $3$ dB off from that at the cell center. 
%As the path loss is almost the same across a cell due to similar path distance from the satellite to the ground, the antenna gain dictates the delivered \snr given the channel gain is common to all users when there is no randomness on the channel.
%However, the shadowing diversifies the delivered \snr on the ground. Especially under a heavy shadowing, \snr is significantly degraded. 
%We compare \cdf of \snr under various shadowing level with elevation angle $90^\circ$ and $45^\circ$ in \figref{fig:snr_el} to see the impact of elevation angle to \snr distribution. 
%
%we compare \cdf of \snr with elevation angle $90^\circ$ and $45^\circ$. In the figure, solid lines and dotted lines represent the \cdf of \snr under $\epsilon= 90^\circ$ and $\epsilon=45^\circ$, respectively. 
%It is shown that the plots with $\epsilon=45^\circ$ for all shadowing level are shifted left around $2$ to $3$ dB from that with $\epsilon=90^\circ$, which is because of the increased path distance as the elevation angle is off from $90^\circ$. 

\subsection{INR Distribution}

\begin{figure*}[!t]
	\centering
	\subfloat[Elevation of $\epsilon = 90^\circ$.]{\includegraphics[width=0.475\linewidth,height=\textheight,keepaspectratio]{fig/heat_90_inr} \hfill
		\label{fig:inr-90}}
	\subfloat[Elevation of $\epsilon = 45^\circ$.]{\includegraphics[width=0.475\linewidth,height=\textheight,keepaspectratio]{fig/heat_45_inr}\hfill
		\label{fig:inr-45}}\\
	\caption{INR on the ground per elevation angle under a light shadowing with the frequency reuse of one.}
	\label{fig:inr-el}
\end{figure*}

Having considered \gsnr, we now turn our attention to examining \ginr in a similar manner.
In \figref{fig:inr-el}, we plot a realization of \ginr as a function of user location for elevations of $90^\circ$ and $45^\circ$ under light shadowing.
At an elevation of $90^\circ$, \ginr typically ranges from around $10$ dB to upwards of $20$ dB.
Inverse to \gsnr, \ginr tends to increase as users approach the cell edge, where spot beam overlap is at its peak.
At an elevation of $45^\circ$, \ginr increases overall by about $2$--$3$ dB due to the distorted beam gain, whereas \gsnr decreased by about the same amount. 
Interestingly, we see that \ginr tends to be higher in region B compared to region A---also opposite what was observed with \gsnr. 
\edit{This is most easily explained by the fact that BLANK. You say this is due to a difference in the number of dominant interferers, but I'm having trouble reasoning through that.}

Thus far, we have assumed a frequency reuse factor of one.
Unlike \gsnr, \ginr is dictated by the particular frequency reuse factor since inter-beam interference is reduced as frequency reuse is increased.
In \figref{fig:inr-cdf-a}, we plot the \cdf of \ginr for various levels of shadowing and for elevations $\epsilon = 90^\circ$ and $\epsilon = 45^\circ$, where the frequency reuse factor is one.
This is essentially the \cdf of user locations in the center cell in \figref{fig:inr-el}.
In \figref{fig:inr-cdf-b}, we plot that in \figref{fig:inr-cdf-a} except with a frequency reuse factor of three.
\figref{fig:inr-cdf-a} illustrates that increasing the shadowing level reduces interference between spot beams and shows that elevation plays a minor role in overall distribution---approximately a mere $2$--$3$ dB increase from $90^\circ$ to $45^\circ$.
With a frequency reuse factor of three, on the other hand, different conclusions are drawn.
As with a frequency reuse factor of one, overall interference reduces as shadowing intensifies with a frequency reuse factor of three.
Naturally, interference decreases as the frequency reuse factor is increased from one to three---here, by about $15$ dB.
Notice that, with a frequency reuse factor of one, the system tends to be interference-limited ($\minr > 0$ dB), except on occasion under heavy shadowing.
With a frequency reuse factor of three, however, the system is more often noise-limited.
When overhead at elevations close to $90^\circ$, even light shadowing has a median \ginr just less than $0$ dB.
As the elevation drops to $45^\circ$, the \ginr distribution shifts rightward by about $6$--$7$ dB, pushing the system to more often be interference-limited.
This shift in limitedness as the satellite traverses across the sky motivates the design of adaptable \leo satellite systems, which may sway from interference-limited to noise-limited and back to interference-limited within a minute or two.
In addition, these results emphasize that elevation, shadowing intensity, and frequency reuse factor should all be taken into account when evaluating the effects of spot beam interference and its distribution.

% Compared to an elevation of $90^\circ$, the system sees an increases of $6$--$7$ dB in interference at an elevation of $45^\circ$. 

% \edit{Will finish this once we get the new results.}

%Based on \figref{fig:gain-elevation}, it is foreseeable that how the heatmap of large-scale \snr will look at the elevation angle $\epsilon = 90^\circ$ and $\epsilon = 45^\circ$ by \eqref{eq:msnr}. 
%Because of the exceptionally long distance from the satellite to the ground compared to the cell radius, the delivered antenna gain will determine the large-scale SNR across a cell.
%\figref{fig:snr-elevation} presents the heatmap of SNR as a function of user location on the ground under light shadowing. 
%On top of the delivered antenna gain, 
%the channel's randomness seems to play a role in determining the received SNR. 
%Even at $\epsilon=90^\circ$, the distance from the cell center does not dictate the SNR values. Instead, 
%even users around the cell center area can experience relatively poor SNR quality due to shadowing.  
%Also, due to the beam shape 
%at $\epsilon=45^\circ$, users in area B can experience relatively lower SNR values than users in area A. 
%Overall, the range of \snr at $\epsilon=45^\circ$ is reduced $2$ to $3$ dB due to longer distance by the elevation angle. 
%
%We now show the heatmap of \inr across cells as a function of ground user location at the elevation angle of $90^\circ$ and $45^\circ$ in \figref{fig:inr-el}. 
%At $\epsilon = 90^\circ$, we observe relatively higher interference around the cell boundaries and lower interference at cell center areas as expected. 
%On the other hand, with $\epsilon=45^\circ$, not every user around the cell boundaries experiences a similar interference level. 
%Users around area B in \figref{fig:inr-45} tend to experience similar 
%interference levels as those in that area when $\epsilon=90^\circ$. However, users in area A potentially experience less interference than users in area B. 
%It might sound counter-intuitive that users in B experience higher interference than users in A   considering the delivered beam shape at $\epsilon=45^\circ$ \figref{fig:gain-elevation}. However, it can be explained in terms of the number of dominant interferers in each area. 
%In other words, due to the beam steering direction, users in area A can have one dominant interferer while those in area B have at least two dominant interferers at $\epsilon=45^\circ$. 
%Tendencies of \inr heatmap look almost opposite to that of \snr heatmap. 


%We also notice that \inr in this system is quite high ($\gg 0$ dB) even in the cell center area leading the system to operate in an interference-limited regime. 
%This is because the system is under the frequency reuse factor (FRF) of one, where all surrounding cells use the same frequency resources. The cell radius ($10$ km) is decided based on the $3$ dB beamwidth, which means $3$ dB less antenna gain is delivered to the cell boundary than the cell center, as seen in \figref{fig:gain-elevation}. 
%At the same time, due to the smaller separation among antennas on board the satellite, a significant portion of inter-cell interference comes from the main lobes of adjacent spot beams. 
%Therefore, it is inevitable to avoid a very high \inr level when the FRF of 1.
%with FRF of 1. One of the common remedies for this issue is to use less aggressive FRF like $3$. 



%
%How does this distorted beam pattern impact INR?
%How does shadowing impact INR?

\begin{figure*}
	\centering
	\subfloat[Frequency reuse factor of 1.]{\includegraphics[width=0.47\linewidth,height=\textheight,keepaspectratio]{fig/frf1_90_45_inr_v03.eps}
		\label{fig:inr-cdf-a}}
	\hfill
	\subfloat[Frequency reuse factor of 3.]{\includegraphics[width=0.47\linewidth,height=\textheight,keepaspectratio]{fig/frf3_90_45_inr_v02.eps}
		\label{fig:inr-cdf-b}}
	\caption{The \cdf of \ginr for various shadowing levels at elevations of $90^\circ$ and $45^\circ$ with (a) a frequency reuse factor of 1 and (b) a frequency reuse factor of 3.}
	\label{fig:inr-cdf}
\end{figure*}


%\begin{figure*}[!t]
%	\centering
%	\subfloat[INR per elevation angle under FRF of 1. ]{\includegraphics[width=0.5\linewidth]{fig/frf1_90_45_inr} \hfill
%		\label{fig:inr_frf1}}
%	\subfloat[INR per elevation angle under FRF of 3.]{\includegraphics[width=0.5\linewidth]{fig/frf3_90_45_inr}\hfill
%		\label{fig:inr_frf3}}\\
%	\caption{INR on the ground per elevation angle under a light shadowing depending on FRF. }
%	\label{fig:inr_frf}
%\end{figure*}


%\figref{fig:inr_frf} shows the \cdf of \inr with $\epsilon=90^\circ$ and $\epsilon=45^\circ$ in various shadowing levels per the value of FRF. Combining results from Fig.. 7, the shadowing not only decreases \snr as seen in \figref{fig:snr_sh_el} but also reduces \inr. 
%It is clearly shown in \figref{fig:inr_frf1} that the system operates under an interference-limited regime at both elevation angles in the light and average level of shadowing 
%as \inr values are almost always larger than $0$ dB when FRF is 1. 
%Under the heavy shadowing, the system is not perfectly interference-limited, however,  it is mostly interference-limited as $30$ percentage of tale is less than $0$ dB. 
%In the figure, we observe a slight increase of \inr at $\epsilon=45^\circ$ than that at $\epsilon=90^\circ$; however, the increase is marginal. 
%Overall, the system under the FRF of 1 suffers from severe interference without respect to the elevation angle. 
%
%In \figref{fig:inr_frf3}, we show the less aggressive frequency reuse affects on \inr. 
%With the FRF of 3, it is seen that \inr values are decreased significantly for all shadowing levels at $\epsilon=90^\circ$. 
%Though the system is not strictly noise-limited under light and average shadowing, a significant portion of tails of \inr distribution is less than $0$ dB. %; thus, the system will not suffer from severe interference. 
%However, with the elevation angle of $45^\circ$, we observe that the \cdf of \inr in every shadowing level is shifted right, and the system is close to interference-limited under light and average level shadowing. 
%It should be noted that the elevation angle of a satellite is not a static parameter in \leo satellite systems, instead the value is a fast varying depending on the orbiting velocity of the satellite. 
%The system is close to noise-limited as the satellite moves to the right above target users and then interference-limited as it fades away. 
%The transition from the interference-limited to the noise-limited regime and vice versa repeats within a very short time interval, e.g., in the order of several minutes, 
%due to frequent handovers caused by the high orbiting velocity of \leo satellites. 



%a. Show for various elevation angles 
%bundled together under average shadowing, for various FRF
%b. Show for various levels of shadowing for FRF = 1 or 3 or maybe both if not too cluttered at a single elevation angle (90 or 60?)
%
%a. INR does not change much as a function of elevation angle for FRF=1 but does for FRF=3.
%
%a. INR does change a lot for increased FRF and elevation angle has more of an impact for higher FRF.
%
%b. INR does change a lot for various levels of shadowing.

\subsection{SINR Distribution}
To conclude our numerical evaluation, we now examine downlink \gsinr, the chief metric quantifying system performance.

% \edit{Will finish this once we get the new results.}

%\begin{figure*}[!t]
%	\centering
%	\subfloat[SINR distribution per FRF at $\epsilon = 90^\circ$ ]{\includegraphics[width=0.5\linewidth]{fig/frf13_90_sinr} \hfill
%		\label{fig:sinr_frf}}
%	\subfloat[SINR per elevation angle with the FRF of three. ]{\includegraphics[width=0.5\linewidth]{fig/frf3_sinr}\hfill
%		\label{fig:sinr_ele}}\\
%	\caption{SINR distribution on the ground as a function of elevation angle, frequency reuse factor and shadowing level. }
%	\label{fig:sinr_frf_ele}
%\end{figure*}

\begin{figure*}
	\centering
	\subfloat[Caption a.]{\includegraphics[width=0.49\linewidth,height=\textheight,keepaspectratio]{fig/frf13_90_sinr}
		\label{fig:sinr-cdf-a}}
	\hfill
	\subfloat[Caption b.]{\includegraphics[width=0.49\linewidth,height=\textheight,keepaspectratio]{fig/frf3_sinr}
		\label{fig:sinr-cdf-b}}
	\caption{Caption here.}
	\label{fig:sinr-cdf}
\end{figure*}

%We present the \cdf of \sinr as a function of elevation angle, FRF, and shadowing level in \figref{fig:sinr_frf_ele}. We compare the \cdf of \sinr under various shadowing level per the value of FRF in \figref{fig:sinr_frf}. 
%The $50$-percentile \sinr under light and average shadowing level is improved around $10$ dB by the adopting the FRF of 3, and the increase in heavy shadowing is around $5$ dB. 
%As we observed in \figref{fig:inr_frf}, a larger value of FRF suppresses \inr and thus improves \sinr in turn. Note \snr is not affected by the values of FRF. 
%\figref{fig:sinr_ele} illustrates the \cdf of \sinr under various shadowing levels per elevation angle when the FRF is 3. 
%Due to the decrease of \inr at $\epsilon=90^\circ$ with the FRF of 3, we see the enhanced \sinr compared to that with FRF of 1. However, as we observed \inr increase at $\epsilon=45^\circ$ in \figref{fig:inr_frf}, the increased \inr is directly translated into the degradation of \sinr. 
%As \inr is heavily dependent on the elevation angle when the FRF is 3, the \sinr also varies as a function of the elevation angle. \leo satellite communication systems experience time varying \sinr distribution caused by the fast orbiting velocity of \leo satellites. 




